Learning from Humans for Proactive Assistance in Human-Robot Collaborative Transport

We focus on human-robot collaborative transport, a challenging task of broad relevance spanning logistics, manufacturing, and the home, in which a user and a robot work together to relocate a large or heavy object. To act as an effective partner, the robot should reduce the user's effort by contributing to efficient relocation of the object while remaining physically responsive to them. Prior work often addresses these capabilities separately, producing robots that may move the object efficiently but resist user input, or accommodate the user but depend on continuous guidance. Our key insight is that obstacle-constrained collaborative transport requires integrating predictions of human collaborative behavior with compliant robot control. To this end, we introduce PROACT, a framework for human-robot collaborative transport that incorporates anticipation into compliant whole-body control through a learned model of human collaborative behavior. Trained on a large-scale, real-world dataset of dyadic human transport demonstrations, our transformer architecture distills collaborative behavior into predictions of future object motion. Across 108 real-world trials with a 9-DoF mobile manipulator, PROACT reduces mean interaction work by 59.2\% and 20.4\%, and mean completion time by 12.9\% and 6.9\%, relative to compliance-only and MPC baselines, respectively. Footage from our experiments can be found at https://youtu.be/qAGvQfVPjbk.

==> sections/02.1-old-introduction.tex <==

% \cmnote{narrative for intro:
% \begin{itemize}
%     \item 1. rich interest in physical hrc. some prior work exists, but robot is typically treated as a tool that follows the human, rather than a partner; settings are overly simplified; physical interaction is minimal or 0. this is due to both hardware and algorithmic challenges
%     \item 2. elevating robots to true partners requires that robots can understand and react appropriately to human behavior during collaboration. this in turn motivates the development of human models, capable of human behavior prediction. a lot of work exists in human modeling but it is mostly focused on non interactive tasks, like tracking people in sports, human-object interaction, etc.
%     \item 3. part of the reason why there is limited progress on human modeling in physical collaboration is the lack of good datasets. existing datasets lack critical modalities, are short, or feature simplified interaction.
%     \item In this paper, we contribute: 1, 2, 3 (your bullets)
% \end{itemize}
% }

% \cmnote{the role of the related work is to follow this narrative in a more technical, deep fashion}

% Enabling
Although specialized collaborative robots for tasks like surgery~\citep{taylor1999steadyhand,colan2025human} have existed for a few decades, the vision of collaborative robot partners, capable of assisting people in physically demanding everyday-life tasks, remains elusive. 
% \jason{just a random thought --- you might throw in that this everyday life collaborator is in addition to specialized collaborative robots such as the steady hand robot for microsurgical manipulations \url{https://link.springer.com/chapter/10.1007/10704282_112}.}
% driven in part by rapid advancements in hardware for mobile manipulators.
% A particularly challenging task in physical human-robot collaboration is the collaborative transport of large objects.
Despite recent advances in hardware and algorithms, collaborative robotics applications are limited to structured setups such as planar-only transport~\citep{solak2025context,peternel2017comanipulation,ng2023takes,ng2023diffusion,yang2025implicit,dominguez2023improving,dominguez2024exploring,dominguez2024force,mortl2012role}, minimal physical collaboration with humans in simulated environments~\citep{nikolaidis2017human,kucukyilmaz2019online}, or minimal to no autonomy~\citep{ng2023takes,ng2023diffusion}. When autonomy is involved, robots are often passively following the human lead~\citep{bussy2012transportation,bussy2012proactive,mielke2024comanipulation,lima2023assistive,solanes2018human,dominguez2023improving,dominguez2024exploring,dominguez2024force}. %\cmnote{need to rebalance cites to support all points}
 % example, collaborative robots are often completing tasks in parallel to their human partners, 
% directly controlled by a user \elvin{cite}, or 

% Finally, systems are often evaluated under settings involving minimal explicit physical collaboration, or in simulated worlds or using teleoperation.

% \jason{Does the argument here need motivation that this reaction to human behavior must come from general perception and not encumbering the human with onerous widgets, tags, or what have you?  I think this may be the point that sits wrong with me about the abstract -- we jump from collaborative transport being an important task to the main contribution of introducing 3d human pose into the dataset.  why do we need pose?  becausae the robot must be able to understand the human behavior through generic perception.}
Elevating robots to partners on general physical tasks requires that they engage in natural interactions with their human counterparts. Prior work on developing physically collaborative robots often relies on heavy instrumentation, either on the transported object (e.g., force-torque, or IMU sensors~\citep{yacoub2021improving,allen2025comanipulation}) or on the human side (e.g., EMG or force sensors~\citep{peternel2017comanipulation}), and on software interfaces (e.g., augmented or mixed reality~\citep{delmerico2022spatial,walker2023vamsurvey}). This level of instrumentation limits the generality and usability of such solutions, motivating the development of intuitive, physical interfaces that do not overload the user or require tedious workspace preparation. One such paradigm involves the incorporation of human models based on \emph{general perception} through readily available robot sensors like cameras and end-effector force sensors.

In recent years, we have seen tremendous progress on human modeling via general perception by leveraging vision and force information. Approaches encompass simple exemplars of human action~\citep{sadanand2012cvpr} to rich inference of human pose~\citep{wang2024tram,jeong2024multi}, action recognition~\citep{kong2022human}, intent estimation~\citep{hoffman2024inferring}, and multiagent trajectory prediction~\citep{hoffman2024inferring,nayakanti2023wayformer,salzmann2023hst}, and are largely based on data-driven machine learning.




% \jason{I recommend reworking this paragraph.  Two high level comments.  Try to make the first sentence of every paragraph the most important one.  lazy reviewers may only read the first sentence (learned this from Frank Dellaert).  And avoid circular flow, where you bring ideas from the last paragraph back into the discussion but at the end of the new one.  This forces the reviewer to think hard and, reminder, they are lazy.  or at least they are overworked and make their job easy.  Short paragraphs are fine.  Here, there seem to be two main points woven together: 1 there is not too much work in physically grounded collaborative transport; 2 there is no dataset with perceptual underpinning to support that work.  separate these out.}
% Despite progress on human modeling, physically collaborative human behavior modeling has received less attention, despite its broad relevance to many domains. This limited attention is likely due to the challenging multimodal nature of physical tasks, blending together motion, force, vision, and semantic context.
% \cmnote{add 1-2 sentences with refs from related work to support the point, but also acknowledge that some work exists?}
% \elvin{Prior work doesn't do multimodal because it's hard cite cite cit}
%\cmnote{expand by adding a few papers} %\jason{Yes, expand.  But also, language just drops in out of nowhere here.  Do we need to say language?}

Despite this progress on human modeling, physically collaborative human behavior modeling has received less attention, despite its broad relevance to many domains.
A critical reason is the lack of high-quality datasets recording the multimodal nature of physical tasks. Much of the progress in human modeling has been pioneered by data-driven architectures, trained on a wide range of large and well-curated high-fidelity human datasets. To model physically collaborative human behavior with current learning architectures, it is critical to develop datasets of equivalent quality. However, the few existing datasets for collaborative transport tend to omit modalities that are essential for human modeling such as full-body poses~\citep{ng2023takes,ng2023diffusion,freeman2024classification}. Datasets in areas that share some aspects with collaborative transport, such as human-object interaction and human-robot collaboration, commonly track full-body poses but do not involve direct physical collaboration~\citep{bhatnagar2022behave,jiang2023full,zhang2024force,yasar2024posetron}.


% This progress has been made possible thanks to a new class of model architectures \cmnote{cite}, trained across wide range of open datasets of human behavior.

% Much of this work does not consider physically collaborative contexts,
% where the direct and sustained contact of multiple agents imposes constraints on how a human can move and convey their intent.


% Models for human behavior have often been enabled by the availability of large and well-curated datasets.

% In contrast, progress on modeling humans in physically collaborative settings has been limited in part by the lack of suitable datasets.

